Distributed Mapping with Privacy and Communication Constraints: Lightweight Algorithms and Object-based Models

We consider the following problem: a team of robots is deployed in an unknown environment and it has to collaboratively build a map of the area without a reliable infrastructure for communication. The backbone for modern mapping techniques is pose graph optimization, which estimates the trajectory of the robots, from which the map can be easily built. The first contribution of this paper is a set of distributed algorithms for pose graph optimization: rather than sending all sensor data to a remote sensor fusion server, the robots exchange very partial and noisy information to reach an agreement on the pose graph configuration. Our approach can be considered as a distributed implementation of the two-stage approach of Carlone et al., where we use the Successive Over-Relaxation (SOR) and the Jacobi Over-Relaxation (JOR) as workhorses to split the computation among the robots. As a second contribution, we extend %and demonstrate the applicability of the proposed distributed algorithms to work with object-based map models. The use of object-based models avoids the exchange of raw sensor measurements (e.g., point clouds) further reducing the communication burden. Our third contribution is an extensive experimental evaluation of the proposed techniques, including tests in realistic Gazebo simulations and field experiments in a military test facility. Abundant experimental evidence suggests that one of the proposed algorithms (the Distributed Gauss-Seidel method or DGS) has excellent performance. The DGS requires minimal information exchange, has an anytime flavor, scales well to large teams, is robust to noise, and is easy to implement. Our field tests show that the combined use of our distributed algorithms and object-based models reduces the communication requirements by several orders of magnitude and enables distributed mapping with large teams of robots in real-world problems.

==> analysis.tex <==
\section{Appendix: Convergence of Distributed Rotation Estimation}
\label{sec:analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h!]
% \centering%
% \includegraphics[width=\columnwidth]{figures/theorem1} \\
% \caption{\label{fig:analysis}
% from Barooah05icisip
% }
% \vspace{-0.5cm}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this appendix we show that the distributed Jacobi algorithm, applied to 
the linear system 

==> figFactorGraph.tex <==

\vspace{-0.2cm}
\begin{figure}[h]
\centering
\includegraphics[width=0.7\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{figures/factorGraph.jpg} 
\caption{\label{fig:factorGraph} Factor graph representation of Multi-Robot Object based SLAM. $\vxx\of{\alpha}{i}$ and $\vxx\of{\beta}{i}$
denote the poses assumed by robot $\alpha$ and $\beta$ at time $i$ respectively. The 
pose of the $k^{th}$ object in the coordinate frame of 
robot $\alpha$ and $\beta$ is denoted with $\vo\of{\alpha}{k}$ and $\vo\of{\beta}{k}$ respectively. Green dots shows inter-robot factors 
whereas orange and purple dots shows intra-robot factors.}
\end{figure}



==> figFlowchart.tex <==

\begin{figure}[h]
\centering
\includegraphics[width=1.0\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{figures/objectSLAMFlowchart.jpg} 
\caption{\label{fig:flowChart}Flowchart of Object based SLAM}
\vspace{-0.3cm}
\end{figure}



==> figRealExperiment.tex <==

\definecolor{dgreen}{rgb}{0,0.5,0}
\renewcommand{\scaleFig}{0.25}

\begin{figure*}[t]
\begin{minipage}{0.6\columnwidth}%\vspace{-3mm}
\begin{tabular}{cc|cc|cc}%
%%%%%%% FIRST ROW
\begin{minipage}{0.5\columnwidth}%
\centering%
\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/icra_realexperiments/1} 
\end{minipage}
&
\begin{minipage}{0.5\columnwidth}%
\centering%
\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/icra_realexperiments/2} 
\end{minipage}
&
\begin{minipage}{0.5\columnwidth}%
\centering%
\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/icra_realexperiments/3} 
\end{minipage}
&
\begin{minipage}{0.5\columnwidth}%
\centering%
\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/icra_realexperiments/4} 
\end{minipage}
&
\begin{minipage}{0.5\columnwidth}%
\centering%
\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/icra_realexperiments/5} 
\end{minipage}
&
\begin{minipage}{0.5\columnwidth}%
\centering%
\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/icra_realexperiments/6} 
\end{minipage}
\vspace{0.1cm}
\\
\hspace{0.2cm} Distributed & Centralized &  Distributed  & Centralized & Distributed &  Centralized
\\
\end{tabular}
\end{minipage}
\caption{\label{fig:realExperiment} Field tests: estimated trajectories for the distributed Jacobi algorithm and for
the centralized two-stage approach~\cite{Carlone15icra-init3D}. Trajectories of the two robots are shown 
in red and blue, while inter-robot measurements are shown in light gray. 
\vspace{-0.5cm}
}
\end{figure*}

%(b) Shows the trajectory estimated using Centralized Two-Stage algorithm. Gray lines show the communication links. (c) and (d) show the convergence
%of rotation and pose estimation respectively.

%%%%%%% SECOND ROW
%\begin{minipage}{0.48\columnwidth}%
%\centering%
%\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/realexperiments_trace/7} 
%\end{minipage}
%&
%\begin{minipage}{0.48\columnwidth}%
%\centering%
%\includegraphics[width=\columnwidth, trim=0cm 0cm 0cm 0cm,clip]{results/realexperiments_trace/8} 
%\end{minipage}
%\vspace{0.1cm}
%\\
%\hspace{0.2cm}(a) Rotation Estimation & (b) Pose Estimation
%\\


==> implementation.tex <==
%!TEX root = main.tex

\section{Implementation Details}
\label{sec:implementation}

\bit
\item flagged initialization
\item initialization of estimate
\eit

==> multirobotObjectBasedSLAM.tex <==
\section{Dealing With Bandwidth Constraints: Compressing sensor data via High-level Semantic Understanding}

In this section we advocate the use of higher-level map representations as a tool to enable operation in bandwidth-constrained multi robot scenarios.  

Maps augmented with objects provide a number of advantages: objects (including planes and other geometric shapes) can
be represented in a compact manner and provide a richer and human-understandable description of the 
environment. Objects are more discriminative, which helps data association and loop-closure detection.
Finally, object representations reduce the computational complexity of SLAM by reducing the number of variables 
(intuitively, we estimate the pose of few objects rather than the position of several 3D points).
%be represented using a compact representation and provide a richer
%description of the environment. It is simpler to include prior constraints
%at the object level than at the lower feature level. The semantic
%information available for an object provides better cues for data
%association as compared to a 3D point cloud. An object would not be
%represented by a 3D point but rather by a 3D point cloud. Joint optimization
%over all the camera poses and objects is computationally cheaper than
%the joint optimization over all the 3D points and cameras since, as
%there are many fewer objects compared to the number of 3D points in
%a map.


% Reasons for multi robot object-based SLAM
% Integrating object-based SLAM with multi robot mapping framework has complimentary benefits for both of them. 
% Using objects instead of point clouds reduces the communication bandwidth and the memory used by each robot, outputs a 
% human understandable map and improves the robustness for multi robot SLAM. Using multi robot SLAM enables faster object level mapping with 
% computation and storage uniformly divided among all the robots. 

% Reasons for using object in multi robotic scenario
We propose an approach for Multi Robot Object-based SLAM with two distinctive features.
The first is the front-end, which performs accurate object detection using \emph{deep learning}. 
Deep learning provides an effective tool to generalize early work on object-based mapping \cite{Moreno13cvpr}
to a large number of object categories.
The second is the back-end, which implements distributed pose graph optimization using the distributed 
Gauss-Seidel method, described in the previous section. 
We show that the combination of these two techniques
 reduces the memory requirement and information exchange among robots, allows accurate and parsimonious large-scale mapping, 
 and scales to large teams.

\subsection{Technical Approach}
\myparagraph{Problem Statement}
We consider a multi robot system and we denote  
each robot with a Greek letter, such that  the 
set of robots is $\robots =\{\alpha, \beta, \gamma, \ldots\}$.
The goal of each robot is to estimate 
its own trajectory  and the pose of a set of objects in the environment, using local measurements, and 
leveraging occasional communication with other robots. 
We model each trajectory  as a finite set of poses; 
the pose assumed by robot $\alpha$ at time $i$ is denoted with $\vxx\of{\alpha}{i}\in \SEthree$;
when convenient, we write $\vxx\of{\alpha}{i} = (\MR\of{\alpha}{i}, \vt\of{\alpha}{i})$,  making explicit that each pose includes a 
rotation $\MR\of{\alpha}{i} \in \SOthree$, and a position $\vt\of{\alpha}{i} \in \Real{3}$.
 The trajectory of robot $\alpha$ is  $\vxx\of{\alpha}{} = [\vxx\of{\alpha}{1},\vxx\of{\alpha}{2}, \ldots]$. Similarly, 
 %we estimate the 
 %pose for each object; 
 %  are modeled as
 % a finite set of poses; 
 we denote with $\vo\of{\alpha}{k}\in \SEthree$ the pose of the 
 $k^{th}$ object in the coordinate frame of robot $\alpha$ (Fig. \ref{fig:factorGraph}).
 %Since each object is observed by multiple robots it instantiates multiple variables 
 %in the factor graph of Fig. \ref{fig:factorGraph}. %However, when the

\input{figFlowchart}

\myparagraph{Object detection and pose estimation}
Each robot collects RGBD data using a depth camera, and measures its ego-motion 
through wheel odometry. In our approach, each RGB frame (from RGBD) is passed to the YOLO object detector~\cite{Redmon15arxiv}, 
which detects objects at 45 frames per second.
% Each RGB frame (from RGBD) is passed to the YOLO object detector which detects objects in real time at the rate of 45 frames per second \cite{Redmon15arxiv}. 
Compared to object-proposal-based detectors, YOLO is fast, since it avoids the computation burden of extracting object proposals, and is less likely to produce false positives in the background. We fine-tune the YOLO detector on a subset of objects from the \emph{BigBird} dataset \cite{Singh14icra}. The training dataset contains the object images in a clean background taken from different viewpoints and labeled images of the same objects taken by a robot in an indoor environment. During testing, we use a probability threshold of 0.3 to avoid false detections. 

Each detected object bounding box is  segmented using the \emph{organized point cloud segmentation} \cite{Trevor13spme}. The segmented object is matched to the 3D template of the detected object class to estimate its pose. We extract PFHRGB features \cite{Rusu08iros} in the source (object segment) and target (object model) point clouds and register the two point clouds in a Sample Consensus Initial Alignment framework \cite{RusuDoctoralDissertation}. If we have at least 12 inlier correspondences, GICP (generalized iterative closest point \cite{Segal09rss}) is performed to further refine the registration and the final transformation is used as the object pose estimate. If less than 12 inlier correspondences are found, the detection is considered to be a false positive. This two-stage process, verifies the detection both semantically and geometrically.  

\myparagraph{Object-based SLAM}
If object pose estimation is successful, it is data-associated with other instances already present in the map by finding the object landmark having the same category label within $2\sigma$ distance of the newly detected object. If there are multiple objects with the same label within that distance, the newly detected object is matched to the nearest object instance. If there exists no object having the same label, a new object landmark is created. 

Before the first rendezvous event, each robot performs 
standard single-robot SLAM using OmniMapper \cite{Trevor12icra}. 
Both wheel odometry and relative pose measurements to the observed objects 
are fed to the SLAM back-end, which is based on pose graph optimization~\cite{Choudhary16icra}.
%a factor graph optimizer based on GTSAM~\cite{gtsam}.
% Object-Pose factors available during some frames along with wheel odometry available during each frame is used infer its trajectory. 
In particular, if object $k$ at pose $\vo\of{\alpha}{k}$ is seen by the robot $\alpha$ from the pose $\vxx\of{\alpha}{i}$, then an \emph{object-pose} factor is added to the  graph:  
\[
f_{op}\left(\vxx\of{\alpha}{i}, \vo\of{\alpha}{k}, \vzz_{ik}\right) \propto\exp\left(-\frac{1}{2}\|
\text{Log}\left(\vzz_{ik}^{-1}\vxx\of{\alpha}{i}^{-1}\vo\of{\alpha}{k}\right) \|_{\Sigma}^{2}\right)
\]
where $\vzz_{ik}$ is the relative pose estimate returned by the object-pose estimator described above, 
$\Sigma \in \Real{6 \times 6}$ is the corresponding covariance, and $\text{Log}$ is the logarithm map for \SEthree. A flowchart of the SLAM approach is given in Fig. \ref{fig:flowChart}.
%The resulting object-pose factors  along with wheel odometry factors are added to the factor graph.  Fig.  \ref{fig:flowChart}
%shows the flowchart. 

\myparagraph{Robot Communication}
During a rendezvous between robots $\alpha$ and $\beta$, robot  $\alpha$ communicates the category labels (class) and poses (in robot $\alpha$'s frame) of all the detected objects to robot $\beta$. 
We assume that the initial pose of each robot is known to all the robots, hence, 
given the initial pose of robot $\alpha$, robot $\beta$ is able to transform the communicated object 
poses from robot $\alpha$'s frame to its own frame.\footnote{The knowledge of the initial pose is only used to facilitate data association but it is not actually 
used during pose graph optimization. We believe that this assumption can be easily relaxed but 
for space reasons we leave this task to future work.} For each object in the list communicated by 
robot $\alpha$, 
robot $\beta$ finds the nearest object in its map, having the 
%the nearest object among the transformed object poses from robot $\alpha$ having the 
same category label and within $2\sigma$ distance. 
If such an object exists, it is added to the list of \emph{shared} objects: this is the set of objects seen by both robots.
%Using this rule, 
%robot $\beta$ finds the set of \emph{shared} objects: this is the set of objects seen by both robots.
% these is the subset of objects observed by $\beta$ whose class matches one of the object seen by 
% $\alpha$; then robot $\beta$ communicates back 
% the labels and the poses (in $\beta$'s frame) of the shared objects. 

\input{figFactorGraph}

The list of shared objects contains pairs $(\vo\of{\alpha}{k},\vo\of{\beta}{l})$ and informs the 
robots that the poses $\vo\of{\alpha}{k}$ and $\vo\of{\beta}{l}$ correspond to the same physical object, 
observed by the two robots.  
For this reason, in the optimization we enforce that the relative pose between
 $\vo\of{\alpha}{k}$ and $\vo\of{\beta}{l}$  is zero.
 We do that by adding an \emph{object-object} factor to the pose graph 
 for each 
 pair  $(\vo\of{\alpha}{k},\vo\of{\beta}{l})$ in the shared object list:
 %, the robots add  \emph{object-object} factor to the pose graph:
%
% If the object instance $\vo\of{\beta}{k}$ is associated with object instance 
% $\vo\of{\alpha}{k}$, then the object-object communication factor is
\[
f_{oo}\left(\vo\of{\beta}{l}, \vo\of{\alpha}{k}\right) 
\propto\exp\left(-\frac{1}{2}\|\text{Log}\left( \vo\of{\beta}{l}^{-1}  \vo\of{\alpha}{k}\right)\|_{\Lambda}^{2}\right)
\]
where $\Lambda \in \Real{6 \times 6}$ specifies the confidence in the  data association among the shared set of objects. We remark that, while before the first rendezvous the robots $\alpha$ and $\beta$ have 
different reference frames,  the object-object factors enforce both robots to have a single 
shared reference frame, facilitating future data association. 


\myparagraph{Distributed Optimization}
% {\bf Measurements.} 
Overall, our approach uses two types of measurements: intra-robot and inter-robot
 measurements. The \emph{intra-robot measurements} consists of the odometry measurements
 which constrain consecutive robot poses (e.g., $\vxx\of{\alpha}{i}$ and $\vxx\of{\alpha}{i+1}$)  and pose-object measurements which constrains
 robot poses with the corresponding visible object landmarks (e.g., $\vxx\of{\alpha}{i}$ and $\vo\of{\alpha}{k}$). 
The \emph{inter-robot measurements} are the ones relating the objects observed by different robots.
According to our previous terminology, an inter-robot measurement is associated to each pair in the 
shared object list. 
% For instance, during a rendezvous, robot $\alpha$, communicates the set of objects with a second robot $\beta$ and  
% constrains the relative pose between the common set of objects seen by both the robots.
% Therefore, robot $\alpha$ acquires a set of inter-robot measurements, where each measurement describes the relative pose between
% $\vo\of{\alpha}{k}$ and $\vo\of{\beta}{k}$ for the $k^{th}$ object seen by both the robots. 
Fig. \ref{fig:factorGraph}
shows the pose graph containing intra and inter-robot measurements. 
 %\vspace{0.3cm}
 %Let us collect all robot trajectories and objects in a single 
 %(to-be-estimated) set of poses $\vxx = [\vxx\of{\alpha}{}, \vxx\of{\beta}{}, \vxx\of{\gamma}{}, \ldots ]$
 %and set of objects  $\vo = [\vo_1, \vo_2, \ldots, \vo_{k}, \ldots ]$. 
 %The set of all available inter-robot and intra-robot measurements  is denoted by $\vz$.
%The \textbf{ML} estimate for $\vxx$ and $\vo$ is defined as the maximum of the measurement likelihood:
%$\vxx^\star,\vo^\star = \argmax_{\vxx,\vo} \prod \calL( \vz  \;|\; \vxx,\vo)$
%where we assumed independent measurements. 
Given these measurements, we use the
distributed Gauss-Seidel (DGS) algorithm~\cite{Choudhary16icra} to estimate the 3D trajectories of the robots along with the poses of the observed objects. % observed by  the  robots.


==> preamble_symbols.tex <==
%!TEX root = main.tex

% LC: can be inserted
% \newcommand{\qed}{{\hfill $\square$}}

% Format definition
\newrefformat{prob}{Problem\,\ref{#1}}
\newrefformat{def}{Definition\,\ref{#1}}
\newrefformat{sec}{Section\,\ref{#1}}
\newrefformat{sub}{Section\,\ref{#1}}
\newrefformat{prop}{Proposition\,\ref{#1}}
\newrefformat{app}{Appendix\,\ref{#1}}
\newrefformat{alg}{Algorithm\,\ref{#1}}
\newrefformat{cor}{Corollary\,\ref{#1}}
\newrefformat{thm}{Theorem\,\ref{#1}}
\newrefformat{lem}{Lemma\,\ref{#1}}
\newrefformat{fig}{Fig.\,\ref{#1}}
\newrefformat{tab}{Table\,\ref{#1}}

% Problem environment
\newtheorem{theorem}{Theorem}
\newtheorem{problem}{Problem}
\newtheorem{trule}[theorem]{Rule}
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{algorithm}{Algorithm}
%\newtheorem{procedure}{\textbf{Procedure}}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}

% Shortcuts
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\Figure}{Fig.}
\newcommand{\bdmath}{\begin{dmath}}
\newcommand{\edmath}{\end{dmath}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beal}{\beq \begin{array}{ll}}
\newcommand{\eeal}{\end{array} \eeq}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\expl}[1]{&&\qquad\text{\color{gray}(#1)}\nonumber}

% \newcommand{\insertproof}[1]{%
%     % lem:name -> proof_lem_name.tex
%     \StrSubstitute{#1}{:}{_}[\name] % replace : with _
%     \begin{IEEEproof} %\color[rgb]{0.8,0.8,0.8}
%     \input{proof_\name.tex}
%     \end{IEEEproof}
% }

% Calligraphic fonts
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calZ}{{\cal Z}}

% SETS:
\newcommand{\setA}{\textsf{A}}
\newcommand{\setB}{\textsf{B}}
\newcommand{\setC}{\textsf{C}}
\newcommand{\setD}{\textsf{D}}
\newcommand{\setE}{\textsf{E}}
\newcommand{\setF}{\textsf{F}}
\newcommand{\setG}{\textsf{G}}
\newcommand{\setH}{\textsf{H}}
\newcommand{\setI}{\textsf{I}}
\newcommand{\setJ}{\textsf{J}}
\newcommand{\setL}{\textsf{L}}
\newcommand{\setM}{\textsf{M}}
\newcommand{\setN}{\textsf{N}}
\newcommand{\setO}{\textsf{O}}
\newcommand{\setP}{\textsf{P}}
\newcommand{\setQ}{\textsf{Q}}
\newcommand{\setR}{\textsf{R}}
\newcommand{\setS}{\textsf{S}}
\newcommand{\setT}{\textsf{T}}
\newcommand{\setU}{\textsf{U}}
\newcommand{\setV}{\textsf{V}}
\newcommand{\setX}{\textsf{X}}
\newcommand{\setY}{\textsf{Y}}
\newcommand{\setZ}{\textsf{Z}}

%General
\newcommand{\smallheading}[1]{\textit{#1}: }
\newcommand{\algostep}[1]{{\small\texttt{#1:}}\xspace}
\newcommand{\etal}{\emph{et~al.}\xspace}
\newcommand{\setal}{~\emph{et~al.}\xspace}
%\newcommand{\email}[1]{{\smaller \textsf{#1}}}

%Typography
\newcommand{\M}[1]{{\bm #1}} % Face for matrices
\renewcommand{\boldsymbol}[1]{{\bm #1}}
\newcommand{\algoname}[1]{\textsc{#1}} % Name of algorithms

%Editing
\newcommand{\towrite}{{\color{red} To write}\xspace}
\newcommand{\xxx}{{\color{red} XXX}\xspace}
\newcommand{\AC}[1]{{\color{red} \textbf{AC}: #1}}
\newcommand{\LC}[1]{{\color{red} \textbf{LC}: #1}}
\newcommand{\FM}[1]{{\color{red} \textbf{FM}: #1}}
\newcommand{\RT}[1]{{\color{blue} \textbf{RT}: #1}}
\newcommand{\hide}[1]{}
\newcommand{\wrt}{w.r.t.\xspace}
\newcommand{\highlight}[1]{{\color{red} #1}}
\newcommand{\tocheck}[1]{{\color{brown} #1}}
\newcommand{\grayout}[1]{{\color{gray} #1}}
\newcommand{\grayText}[1]{{\color{gray} \text{#1} }}
\newcommand{\grayMath}[1]{{\color{gray} #1 }}
\newcommand{\hiddenText}{{\color{gray} hidden text.}}
\newcommand{\hideWithText}[1]{\hiddenText}


\newcommand{\NA}{{\sf n/a}}
\newcommand{\versus}{\scenario{VS}\xspace}

%Basic math symbols
\newcommand{\kron}{\otimes}
\newcommand{\dist}{\mathbf{dist}}
\newcommand{\iter}{\! \rm{iter.} \;}
\newcommand{\leqt}{\!\!\! < \!\!\!}
\newcommand{\geqt}{\!\!\! > \!\!\!}
\newcommand{\mysetminus}{-} % One set minus another
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\Int}[1]{ { {\mathbb Z}^{#1} } }
\newcommand{\Complex}[1]{ { {\mathbb C}^{#1} } }
\newcommand{\one}{ {\mathbf{1}} }
\newcommand{\subject}{\text{ subject to }}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%% Norms
\newcommand{\normsq}[2]{\left\|#1\right\|^2_{#2}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\normsqs}[2]{\|#1\|^2_{#2}}
\newcommand{\infnorm}[1]{\|#1\|_{\infty}}
\newcommand{\zeronorm}[1]{\|#1\|_{0}}
\newcommand{\onenorm}[1]{\|#1\|_{1}}
\newcommand{\lzero}{\ell_{0}}
\newcommand{\lone}{\ell_{1}}
\newcommand{\linf}{\ell_{\infty}}

\newcommand{\E}{{\mathbb{E}}}
\newcommand{\EV}{\mathbb{E}}
\newcommand{\erf}{{\mathbf{erf}}}
\newcommand{\prob}[1]{{\mathbb P}\left(#1\right)}
% \newcommand{\tran}{^{\top}}
\newcommand{\tran}{^{\mathsf{T}}}
\newcommand{\traninv}{^{-\mathsf{T}}}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\trace}[1]{\mathrm{tr}\left(#1\right)}
\newcommand{\conv}[1]{\mathrm{conv}\left(#1\right)}
\newcommand{\polar}[1]{\mathrm{polar}\left(#1\right)}
\newcommand{\rank}[1]{\mathrm{rank}\left(#1\right)}
\newcommand{\e}{{\mathrm e}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^\dag}
\newcommand{\until}[1]{\{1,\dots, #1\}}
\newcommand{\ones}{{\mathbf 1}}
\newcommand{\zero}{{\mathbf 0}}
\newcommand{\eye}{{\mathbf I}}
\newcommand{\vect}[1]{\left[\begin{array}{c}  #1  \end{array}\right]}
\newcommand{\matTwo}[1]{\left[\begin{array}{cc}  #1  \end{array}\right]}
\newcommand{\dss}{\displaystyle}
\newcommand{\Real}[1]{ { {\mathbb R}^{#1} } }
\newcommand{\reals}{\Real{}}
\newcommand{\opt}{^{\star}}
\newcommand{\only}{^{\alpha}}
\newcommand{\copt}{^{\text{c}\star}}
\newcommand{\atk}{^{(k)}}
\newcommand{\att}{^{(t)}}
\newcommand{\at}[1]{^{(#1)}}
\newcommand{\attau}{^{(\tau)}}
\newcommand{\atc}[1]{^{(#1)}}
\newcommand{\atK}{^{(K)}}
\newcommand{\atj}{^{(j)}}
\newcommand{\projector}{{\tt projector}}
\newcommand{\setdef}[2]{ \{#1 \; {:} \; #2 \} }
\newcommand{\smalleye}{\left(\begin{smallmatrix}1&0\\0&1\end{smallmatrix}\right)}

%Spaces
\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}\xspace}
\newcommand{\SE}[1]{\ensuremath{\mathrm{SE}(#1)}\xspace}
\newcommand{\SEthree}{\ensuremath{\mathrm{SE}(3)}\xspace}
\newcommand{\SOtwo}{\ensuremath{\mathrm{SO}(2)}\xspace}
\newcommand{\SOthree}{\ensuremath{\mathrm{SO}(3)}\xspace}
\newcommand{\Othree}{\ensuremath{\mathrm{O}(3)}\xspace}
\newcommand{\SOn}{\ensuremath{\mathrm{SO}(n)}\xspace}
\newcommand{\SO}[1]{\ensuremath{\mathrm{SO}(#1)}\xspace}
\newcommand{\On}{\ensuremath{\mathrm{O}(n)}\xspace}
\newcommand{\sotwo}{\ensuremath{\mathrm{so}(2)}\xspace}
\newcommand{\sothree}{\ensuremath{\mathrm{so}(3)}\xspace}
\newcommand{\intexpmap}[1]{\mathrm{Exp}\left(#1\right)}
\newcommand{\intlogmap}[1]{\mathrm{Log}\left(#1\right)}
\newcommand{\logmapz}[1]{\mathrm{Log}_0(#1)}
\newcommand{\loglikelihood}{\mathrm{log}\calL}
\newcommand{\intprinlogmap}{\mathrm{Log}_0}
\newcommand{\expmap}[1]{\intexpmap{#1}}
\newcommand{\expmaps}[1]{\langle #1 \rangle_{2\pi}}
\newcommand{\biggexpmap}[1]{\left\langle #1 \right\rangle_{2\pi}}
\newcommand{\logmap}[1]{\intlogmap{#1}}
\newcommand{\round}[1]{\mathrm{round}\left( #1 \right)}

% Matrices 
\newcommand{\MA}{\M{A}}
\newcommand{\MB}{\M{B}}
\newcommand{\MC}{\M{C}}
\newcommand{\MD}{\M{D}}
\newcommand{\ME}{\M{E}}
\newcommand{\MJ}{\M{J}}
\newcommand{\MK}{\M{K}}
\newcommand{\MG}{\M{G}}
\newcommand{\MM}{\M{M}}
\newcommand{\MN}{\M{N}}
\newcommand{\MP}{\M{P}}
\newcommand{\MQ}{\M{Q}}
\newcommand{\MU}{\M{U}}
\newcommand{\MR}{\M{R}}
\newcommand{\MS}{\M{S}}
\newcommand{\MI}{\M{I}}
\newcommand{\MV}{\M{V}}
\newcommand{\MF}{\M{F}}
\newcommand{\MH}{\M{H}}
\newcommand{\ML}{\M{L}}
\newcommand{\MO}{\M{O}}
\newcommand{\MT}{\M{T}}
\newcommand{\MX}{\M{X}}
\newcommand{\MY}{\M{Y}}
\newcommand{\MW}{\M{W}}
\newcommand{\MZ}{\M{Z}}
\newcommand{\MSigma}{\M{\Sigma}} 
\newcommand{\MOmega}{\M{\Omega}}
\newcommand{\MPhi}{\M{\Phi}}
\newcommand{\MPsi}{\M{\Psi}}
\newcommand{\MLambda}{\M{\Lambda}}

% vectors
\newcommand{\va}{\boldsymbol{a}} 
\newcommand{\vb}{\boldsymbol{b}}
\newcommand{\vc}{\boldsymbol{c}}
\newcommand{\vd}{\boldsymbol{d}}
\newcommand{\ve}{\boldsymbol{e}}
\newcommand{\vf}{\boldsymbol{f}}
\newcommand{\vg}{\boldsymbol{g}}
\newcommand{\vk}{\boldsymbol{k}}
\newcommand{\vn}{\boldsymbol{n}}
\newcommand{\vo}{\boldsymbol{o}}
\newcommand{\vp}{\boldsymbol{p}}
\newcommand{\vq}{\boldsymbol{q}}
\newcommand{\vr}{\boldsymbol{r}}
\newcommand{\vs}{\boldsymbol{s}}
\newcommand{\vu}{\boldsymbol{u}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\vt}{\boldsymbol{t}}
\newcommand{\vxx}{\boldsymbol{x}} 
\newcommand{\vy}{\boldsymbol{y}}
\newcommand{\vw}{\boldsymbol{w}}
\newcommand{\vzz}{\boldsymbol{z}} 
\newcommand{\vdelta}{\boldsymbol{\delta}}
\newcommand{\vgamma}{\boldsymbol{\gamma}}  
\newcommand{\vlambda}{\boldsymbol{\lambda}}
\newcommand{\vtheta}{\boldsymbol{\theta}}
\newcommand{\vnu}{\boldsymbol{\nu}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vepsilon}{\boldsymbol{\epsilon}}

%Intrinsic geometry
\newcommand{\Rtheta}{\boldsymbol{R}}
\newcommand{\symf}{f} % Symmetry function

%Angles
\newcommand{\angledomain}{(-\pi,+\pi]}

% Tree, graphs, and cycle basis
\newcommand{\MCB}{\mathsf{MCB}}
\newcommand{\FCM}{\mathsf{FCM}}
\newcommand{\FCB}{\mathsf{FCB}}
\newcommand{\cyclemap}[1]{\calC^{\calG}\left(#1\right)}
\newcommand{\incidencemap}[1]{\calA^{\calG}\left(#1\right)}
\newcommand{\cyclemapk}{\calC^{\calG}_{k}}
\newcommand{\incidencemapij}{\calA^{\calG}_{ij}}
\renewcommand{\ij}{_{ij}}

\newcommand{\foralledges}{\forall(i,j) \in \calE}

\newcommand{\sumalledges}{
     \displaystyle
     \sum_{(i,j) \in \calE}}
     
\newcommand{\sumalledgesm}{
     \displaystyle
     \sum_{i=1}^{m}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\To}{\T_{\rm o}}
\newcommand{\Tm}{\T_{\rm m}}
\newcommand{\MCBa}{\MCB_{\mathsf{a}}}
\newcommand{\FCBo}{\FCB_{\mathsf{o}}}
\newcommand{\FCBm}{\FCB_{\mathsf{m}}}

% Algorithms
\newcommand{\algoonlyname}{MOLE2D}
\newcommand{\algoml}{{\smaller\sf \algoonlyname}\xspace}
\newcommand{\algocyclebasis}{\algoname{compute-cycle-basis}}
\newcommand{\scenario}[1]{{\smaller \sf#1}\xspace}
\newcommand{\toro}{{\smaller\sf Toro}\xspace}
\newcommand{\gtwoo}{{\smaller\sf g2o}\xspace}
\newcommand{\gtwooST}{{\smaller\sf g2oST}\xspace}
\newcommand{\gtwood}{{\smaller\sf g2o{10}}\xspace}
\newcommand{\gtsam}{{\smaller\sf gtsam}\xspace}
\newcommand{\isam}{{\smaller\sf iSAM}\xspace}
\newcommand{\lago}{{\smaller\sf LAGO}\xspace}
\newcommand{\egtwoo}{{\smaller\sf \algoonlyname+g2o}\xspace}

% Datasets
\newcommand{\grid}{\scenario{cube}}
\newcommand{\rim}{\scenario{rim}}
\newcommand{\cubicle}{\scenario{cubicle}}
\newcommand{\sphere}{\scenario{sphere}}
\newcommand{\sphereHard}{\scenario{sphere-a}}
\newcommand{\garage}{\scenario{garage}}
\newcommand{\torus}{\scenario{torus}}
\newcommand{\oneloop}{\scenario{circle}}
\newcommand{\intel}{\scenario{INTEL}}
\newcommand{\bovisa}{\scenario{Bovisa}}
\newcommand{\bov}{\scenario{B25b}}
\newcommand{\fra}{\scenario{FR079}}
\newcommand{\frb}{\scenario{FRH}}
\newcommand{\csail}{\scenario{CSAIL}}
\newcommand{\Ma}{\scenario{M3500}}
\newcommand{\Mb}{\scenario{M10000}}
\newcommand{\ATE}{\scenario{ATE}}
\newcommand{\CVX}{\scenario{CVX}}
\newcommand{\NEOS}{\scenario{NEOS}}
\newcommand{\sdptThree}{\scenario{sdpt3}}
\newcommand{\MOSEK}{\scenario{MOSEK}}
\newcommand{\NESTA}{\scenario{NESTA}}
\newcommand{\vertigo}{\scenario{Vertigo}}
\newcommand{\SDPA}{\scenario{SDPA}}

% \newcommand{\tablabel}[1]{%
%     \hspace{-1mm}%
%     \begin{sideways}{\small\scenario{#1}}\end{sideways}%
%     \hspace{-4mm}%
% }
%
% \newcommand{\tabfig}[2]{%
%     \subfloat[\label{fig:#2} #1]{%
%     \begin{minipage}{5.5cm}%
%     \centering%
%     \includegraphics[width=5.5cm,trim=4 0 4 15]{figures/#2}
%     \end{minipage}%
%     }%
% }
%
% \newcommand{\subFigure}[3]{%
%     \subfloat[\label{fig:#2} #1]{%
%     \begin{minipage}{#3cm}%
%     \centering%
%     \includegraphics[width=#3cm,trim=4 0 4 15]{figures/#2}
%     \end{minipage}%
%     }%
% }


\newcommand{\cvx}{{\sf cvx}\xspace}

% PAPER-SPECIFIC COMMANDS
%============================================================================

% Linear approximation
\newcommand{\vpose}{\boldsymbol{x}}
\newcommand{\vz}{\boldsymbol{z}}
\newcommand{\vDelta}{\boldsymbol{\Delta}}
\newcommand{\vposesub}{\hat{\vpose}}
\newcommand{\vpossub}{\hat{\vpos}}
\newcommand{\vthetasub}{\hat{\vtheta}}
\newcommand{\Pthetasub}{\MP_\vtheta}
\newcommand{\thetasub}{\hat{\theta}}
\newcommand{\vposecorr}{\tilde{\vpose}}
\newcommand{\vposcorr}{\tilde{\vpos}}
\newcommand{\vthetacorr}{\tilde{\vtheta}}
\newcommand{\vposestar}{{\vpose}^{\star}}
\newcommand{\vposstar}{{\vpos}^{\star}}
\newcommand{\vthetastar}{{\vtheta}^{\star}}
\newcommand{\vcthetastar}{{\vctheta}^{\star}}
\newcommand{\pose}{\boldsymbol{x}}
\newcommand{\pos}{\boldsymbol{p}}
\newcommand{\mease}{z} % element
\newcommand{\meas}{\boldsymbol{z}} % vector
\newcommand{\meashat}{\hat{\meas}}




